PanelPRO: A R package for multi-syndrome, multi-gene risk modeling for individuals with a family history of cancer

Identifying individuals who are at high risk of cancer due to inherited germline mutations is critical for effective implementation of personalized prevention strategies. Most existing models to identify these individuals focus on specific syndromes by including family and personal history for a small number of cancers. Recent evidence from multi-gene panel testing has shown that many syndromes once thought to be distinct are overlapping, motivating the development of models that incorporate family history information on several cancers and predict mutations for more comprehensive panels of genes. Once such class of models are Mendelian risk prediction models, which use family history information and Mendelian laws of inheritance to estimate the probability of carrying genetic mutations, as well as future risk of developing associated cancers. To flexibly model the complexity of many cancer-mutation associations, we present a new software tool called PanelPRO, a R package that extends the previously developed BayesMendel R package to user-selected lists of susceptibility genes and associated cancers. The model identifies individuals at an increased risk of carrying cancer susceptibility gene mutations and predicts future risk of developing hereditary cancers associated with those genes. Additional functionalities adjust for prophylactic interventions, known genetic testing results, and risk modifiers such as race and ancestry. The package comes with a customizable database with default parameter values estimated from published studies. The PanelPRO package is open-source and provides a fast and flexible back-end for multi-gene, multi-cancer risk modeling with pedigree data. The software enables the identification of high-risk individuals, which will have an impact on personalized prevention strategies for cancer and individualized decision making about genetic testing.

==> archive/0_0performance.tex <==
\section{Package performance}
\label{sec:rcpp_performation}

As we anticipate many more genes to be added to \textbf{PanelPRO}, it is important to ensure that run-times are feasible, especially in clinical contexts. To this end, the peeling-paring algorithm has been written in \Cppspace with the \textbf{Rcpp} and \textbf{RcppArmadillo} packages. In Figure \ref{fig:rcpp_performance} we show relative run-times of the package against an equivalent implementation  (in terms of correctness) which was written solely in \R. The relative run-times compared between the \Rspace and \textbf{Rcpp} implementation, which will become important for larger gene models. We also illustrate the effect of changing the paring parameter from 2 to 3 (the number of simultaneous gene mutations). The run times were tested on a Windows Intel Core i7-4500U CPU (2 cores with 4 logical processors) with a base speed of 1.80GHz and 8GB RAM. The pedigree tested was the \code{small.fam} sample family, which consists of 19 people. The abbreviations in Figure \ref{fig:rcpp_performance} are noted in Table \ref{tab:specifications}.

\begin{table}
	\begin{tabularx}{\linewidth}{XXX}
		\toprule
		Implementation & Parallelized & Sequential \\
		\midrule
		\Rspace & RParallel & RSeq \\
		\textbf{Rcpp} & RcppParallel & RcppSeq \\
		\bottomrule
	\end{tabularx}
	\vspace{0.1cm}
	\caption{References for the different implementations benchmarked.}
	\label{tab:specifications}
\end{table}

\begin{figure}

\begin{tabular}{C{.5\textwidth}C{.5\textwidth}}
%%%%%%%%%%%%%%%%%%%%%% 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfigure [$T = 2$ absolute run times] {
    \resizebox{0.45\textwidth}{!}{%
	\begin{tikzpicture}
	\begin{axis}[%
	            table/col sep=comma,
                % width=5cm,
                height=5cm,
                scale only axis,
                xmin=1, xmax=11,
                xtick={1,2,3,4,5,6,7,8,9,10,11},
                % xticklabels={},
                xmajorgrids,
                xlabel={Number of genes considered},
                ymin=0.0, ymax=12,
                ylabel={Run time (s)},
                ymajorgrids,
                % title={Stroke Ratio Comparison},
                axis lines*=left,
                line width=1.0pt,
                mark size=2.0pt,
                legend style={at={(0.05,0.95)},anchor=north west,draw=black,fill=white,align=left}]
	]
	
	\addplot [color=black,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RcppParallel"}, col sep = comma] {csvs/benchmarks_2_elapsed.csv};
                
	\addplot [color=RoyalPurple,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RcppSeq"}, col sep = comma] {csvs/benchmarks_2_elapsed.csv};
                
    \addplot [color=RoyalBlue,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RParallel"}, col sep = comma] {csvs/benchmarks_2_elapsed.csv};
                
    \addplot [color=ForestGreen,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RSeq"}, col sep = comma] {csvs/benchmarks_2_elapsed.csv};

	\legend{RcppParallel, RcppSeq, RParallel, RSeq}
	
	\end{axis}
	\end{tikzpicture}
    }
} & 
%%%%%%%%%%%%%%%%%%%%%% 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfigure [$T = 3$ absolute run times] {
  \resizebox{0.45\textwidth}{!}{%
    \begin{tikzpicture}
	\begin{axis}[%
	            table/col sep=comma,
                % width=5cm,
                height=5cm,
                scale only axis,
                xmin=1, xmax=11,
                xtick={1,2,3,4,5,6,7,8,9,10,11},
                % xticklabels={},
                xmajorgrids,
                xlabel={Number of genes considered},
                ymin=0.0, ymax=350,
                ylabel={Run time (s)},
                ymajorgrids,
                % title={Stroke Ratio Comparison},
                axis lines*=left,
                line width=1.0pt,
                mark size=2.0pt,
                legend style={at={(0.05,0.95)},anchor=north west,draw=black,fill=white,align=left}]
	]
	
	\addplot [color=black,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RcppParallel"}, col sep = comma] {csvs/benchmarks_3_elapsed.csv};
                
	\addplot [color=RoyalPurple,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RcppSeq"}, col sep = comma] {csvs/benchmarks_3_elapsed.csv};
                
    \addplot [color=RoyalBlue,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RParallel"}, col sep = comma] {csvs/benchmarks_3_elapsed.csv};
                
    \addplot [color=ForestGreen,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {"nGenes"}, y = {"RSeq"}, col sep = comma] {csvs/benchmarks_3_elapsed.csv};

	\legend{RcppParallel, RcppSeq, RParallel, RSeq}
	
	\end{axis}
	\end{tikzpicture}
    }
} \\

%%%%%%%%%%%%%%%%%%%%%% 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfigure [$T = 2$ relative run times] {
  \resizebox{0.45\textwidth}{!}{%
    \begin{tikzpicture}
	\begin{axis}[%
	            table/col sep=comma,
                % width=5cm,
                height=5cm,
                scale only axis,
                xmin=1, xmax=11,
                xtick={1,2,3,4,5,6,7,8,9,10,11},
                % xticklabels={},
                xmajorgrids,
                xlabel={Number of genes considered},
                ymin=0.0, ymax=15,
                ylabel={Relative run times},
                ymajorgrids,
                % title={Stroke Ratio Comparison},
                axis lines*=left,
                line width=1.0pt,
                mark size=2.0pt,
                legend style={at={(0.05,0.95)},anchor=north west,draw=black,fill=white,align=left}]
	]
	
	\addplot [color=black,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RcppParallel}, col sep = comma] {csvs/benchmarks_2_relative.csv};
                
	\addplot [color=RoyalPurple,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RcppSeq}, col sep = comma] {csvs/benchmarks_2_relative.csv};
                
    \addplot [color=RoyalBlue,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RParallel}, col sep = comma] {csvs/benchmarks_2_relative.csv};
                
    \addplot [color=ForestGreen,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RSeq}, col sep = comma] {csvs/benchmarks_2_relative.csv};

	\legend{RcppParallel, RcppSeq, RParallel, RSeq}
	
	\end{axis}
	\end{tikzpicture}
  }
} & 

%%%%%%%%%%%%%%%%%%%%%% 4 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subfigure [$T=3$ relative run times] {
  \resizebox{0.45\textwidth}{!}{%
    \begin{tikzpicture}
	\begin{axis}[%
	            table/col sep=comma,
                % width=5cm,
                height=5cm,
                scale only axis,
                xmin=1, xmax=11,
                xtick={1,2,3,4,5,6,7,8,9,10,11},
                % xticklabels={},
                xmajorgrids,
                xlabel={Number of genes considered},
                ymin=0.0, ymax=20,
                ylabel={Relative run times},
                ymajorgrids,
                % title={Stroke Ratio Comparison},
                axis lines*=left,
                line width=1.0pt,
                mark size=2.0pt,
                legend style={at={(0.05,0.95)},anchor=north west,draw=black,fill=white,align=left}]
	]
	
	\addplot [color=black,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RcppParallel}, col sep = comma] {csvs/benchmarks_3_relative.csv};
                
	\addplot [color=RoyalPurple,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RcppSeq}, col sep = comma] {csvs/benchmarks_3_relative.csv};
                
    \addplot [color=RoyalBlue,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RParallel}, col sep = comma] {csvs/benchmarks_3_relative.csv};
                
    \addplot [color=ForestGreen,
                solid,
                mark=*,
                mark options={solid},
                smooth
                ] table [x = {nGenes}, y = {RSeq}, col sep = comma] {csvs/benchmarks_3_relative.csv};

	\legend{RcppParallel, RcppSeq, RParallel, RSeq}
	
	\end{axis}
	\end{tikzpicture}
    }
} \\
\end{tabular}
\caption{Performance between \R, \textbf{Rcpp} implementations, averaged over 10 iterations. $T$ is the maximum number of simultaneous mutations parameter. For missing current or cancer ages, 10 imputations were done. Relative performance is relative to the line $y=1$.}
\label{fig:rcpp_performance}
\end{figure}

We see that for a low number of genes, at $T=2$, the \textbf{Rcpp} implementation runs in around 2 seconds, whilst the \Rspace implementation runs in just over 10 seconds. Whilst these run-times are feasible, the gains in relative speed of the \textbf{Rcpp} implementation are clearly seen in the $T=3$ run. There are 67 and 232 genotypes in each of these cases, respectively. For comparison, when $K=25$, there are 326 genotypes when $T=2$ and 2,626 when $T=3$. We can thus expect that the run-times for the cases when $(K, T) = (25, 2)$ and $(K, T) = (11, 3)$ are comparable, giving us an idea of how run-times would scale when the database expands to around $K=25$.

==> archive/archive.tex <==
% There is one example pedigree in this package called \code{small.fam}.

% %"mystyle" code listing set
% \lstset{style=mystyle}
% \begin{lstlisting}[language=R, caption=pedigree example]
% > data("small.fam")
% > str(small.fam)
% 'data.frame':	19 obs. of  25 variables:
%  $ ID       : int  1 2 3 4 5 6 7 8 9 10 ...
%  $ Sex      : num  0 1 0 1 1 1 0 1 0 0 ...
%  $ MotherID : num  NA NA 1 1 1 1 NA NA 7 7 ...
%  $ FatherID : num  NA NA 2 2 2 2 NA NA 8 8 ...
%  $ isProband: num  0 0 0 0 1 0 0 0 0 0 ...
%  $ CurAge   : num  93 80 72 65 65 NA 73 75 69 NA ...
%  $ isAffBC  : num  0 0 1 0 0 0 0 0 0 1 ...
%  $ isAffOC  : num  0 0 1 0 0 0 0 0 1 0 ...
%  $ AgeBC    : num  NA NA 40 NA NA NA NA NA NA NA ...
%  $ AgeOC    : logi  NA NA NA NA NA NA ...
%  $ isDead   : num  1 1 0 1 0 0 1 1 0 0 ...
%  $ race     : chr  "All_Races" "All_Races" "All_Races" "whatever" ...
%  $ riskmod  :List of 19
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr "Mastectomy"
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr "Hysterectomy"
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr  "Mastectomy" "Hysterectomy"
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%   ..$ : chr 
%  $ interAge :List of 19
%   ..$ : int 
%   ..$ : int 
%   ..$ : int 28
%   ..$ : int 
%   ..$ : int 
%   ..$ : int 48
%   ..$ : int 
%   ..$ : int 
%   ..$ : int 
%   ..$ : int  27 52
%   ..$ : int 
%   ..$ : int 
%   ..$ : int 
%   ..$ : chr 
%   ..$ : int 
%   ..$ : chr 
%   ..$ : int 
%   ..$ : chr 
%   ..$ : chr 
%  $ Twins    : num  0 0 0 1 1 0 0 0 0 0 ...
%  $ BRCA1    : num  NA 1 NA 0 NA NA NA NA NA 1 ...
%  $ BRCA2    : num  NA 0 NA 1 NA NA NA NA NA 0 ...
%  $ ER       : num  NA NA NA NA NA 0 NA NA NA NA ...
%  $ CK5.6    : num  NA NA NA NA NA NA NA NA NA NA ...
%  $ CK14     : num  NA NA NA NA NA NA NA NA NA NA ...
%  $ PR       : num  NA NA NA NA NA NA NA NA NA 1 ...
%  $ HER2     : num  NA NA NA NA NA NA NA NA NA NA ...
%  $ isAffCBC : num  0 0 1 0 0 0 0 0 0 0 ...
%  $ AgeCBC   : logi  NA NA NA NA NA NA ...
%  $ Ancestry : chr  "nonAJ" "nonAJ" "AJ" "nonAJ" ...
% \end{lstlisting}



% \begin{longtable}{ |p{3cm}||p{8cm}|p{4cm}| }
%  \hline
%  \multicolumn{3}{|c|}{Pedigree}\\
%  \hline
%  Column &Definition &Value\\
%  \hline
%  \code{ID}   & the unique numeric identifier of each individual    & {Non-repeating interger larger than zero}\\
%  \hline
%  \code{MotherID} &   The ID of one's mother  &  {an integer}\\
%  \hline
%  \code{FatherID} & The ID of one's father & {an integer}\\
%  \hline
%  \code{Sex}    & The Sex of each individual, 1 for male, 0 for female  & {One from 0 / 1 / \code{NA}}\\
%  \hline
%  \code{isProband}    &Whether an individual is proband & {One from 0/1}\\
%  \hline
%  \code{CurAge}& Age of censoring: Either of current age or death age depending on \code{isDead} status & {Integer / \code{NA}}   \\
%  \hline
%  \code{isAff*}& affection status of cancer {*}, where {*} can be one of {\code{ "BRA", "BC", "OC", "COL", "ENDO", "GAS",  "KID",  "MELA", "OC",  "PANC", "PROS", "SMA", "CBC"}} that encodes for { \code{"Brain", "Breast", "Colorectal", "Endometrial",   "Gastric","Kidney","Melanoma", "Ovarian", "Pancreas", "Prostate", "Small intestine", "Contralateral"} } cancer  & {0/1}\\
%  \hline
%  \code{Age*}& affection age of cancer {*}, where {*} can be one of {\code{ "BRA", "BC", "OC", "COL", "ENDO", "GAS",  "KID",  "MELA", "OC",   "PANC", "PROS", "SMA", "CBC"}} that encodes for { \code{"Brain", "Breast", "Colorectal", "Endometrial",   "Gastric","Kidney","Melanoma", "Ovarian", "Pancreas", "Prostate", "Small intestine", "Contralateral"} } cancer  & Integer /\code{NA}\\
%  \hline
%  \code{isDead}& Whether someone has died  & {0/1/\code{NA}}\\
%  \hline
%  \code{race} & Race of one individual that modifies penetrance & One from { \code{"All\_Races", "AIAN","Asian", "Black", "White", "Hispanic", "WH", "WNH"}} \\
%  \hline
%  \code{Ancestry} & Ancestry of one individual that modifies prevalence & One from { \code{"AJ", "nonAJ", "Italian"}} \\
%  \hline
%  \code{riskmod} & Preventative interventions that modifies penetrance & List, can be some combination of \code{"Mastectomy"   "Hysterectomy" "Oophorectomy"} \\
%  \hline
%  \code{InterAge} & Age of each preventative interventions & List, can be some combination of integers, the order should agree with \code{riskmod} \\
%  \hline
%  Gene name from \code{PanelPRO:::GENE\_TYPES} & Germline testing result & {One from 0 / 1 / \code{NA}} \\
%  \hline
%  Marker name from \code{"CK14", "CK5.6", "ER", "PR", "HER2", "MSI"} & Marker testing result & {One from 0 / 1 / \code{NA}} \\
%  \hline
 
%  \caption{\label{tab:Table 1}Pedigree structure.}
% \end{longtable}
